Non-Local Cell Adhesion Models: Steady States and Bifurcations

In this manuscript, we consider the modelling of cellular adhesions, which is a key interaction between biological cells. Continuum models of the diffusion-advection-reaction type have long been used in tissue modelling. In 2006, Armstrong, Painter, and Sherratt proposed an extension to take adhesion effects into account. The resulting equation is a non-local advection-diffusion equation. While immensely successful in applications, the development of mathematical theory pertaining to steady states and pattern formation is lacking. The mathematical analysis of the non-local adhesion model is challenging. In this monograph, we contribute to the analysis of steady states and their bifurcation structure. The importance of steady-states is that these are the patterns observed in nature and tissues (e.g. cell-sorting experiments). In the case of periodic boundary conditions, we combine global bifurcation results pioneered by Rabinowitz, equivariant bifurcation theory, and the mathematical properties (maximum principle) of the non-local term to obtain a global bifurcation result for the branches of non-trivial solutions.

==> preface.tex <==
%-----------------------------------------------------------------------------
% Beginning of preface.tex
%-----------------------------------------------------------------------------
%
% AMS-LaTeX 1.2 sample file for a monograph, based on amsbook.cls.
% This is a data file input by chapter.tex.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\chapter*{Preface}

This document is a sample prepared to illustrate the use of the
American Mathematical Society's \LaTeX{} document class
\texttt{amsbook} and publication-specific variants of that class.

This is an example of an unnumbered chapter which can be used for a Preface
or Foreword.

The purpose of this paper is to establish a relationship between an
infinite-dimensional Grassmannian and arbitrary algebraic vector bundles
of any rank defined over an arbitrary complete irreducible algebraic
curve, which generalizes the known connection between the Grassmannian
and line bundles on algebraic curves.

\aufm{Andreas Buttensch\"{o}n and Thomas Hillen}

%-----------------------------------------------------------------------------
% End of preface.tex
%-----------------------------------------------------------------------------

